Random growth models: shape and convergence rate

Random growth models are fundamental objects in modern probability theory, have given rise to new mathematics, and have numerous applications, including tumor growth and fluid flow in porous media. In this article, we introduce some of the typical models and the basic analytical questions and properties, like existence of asymptotic shapes, fluctuations of infection times, and relations to particle systems. We then specialize to models built on percolation (first-passage percolation and last-passage percolation) and give a self-contained treatment of the shape theorem, the subadditive ergodic theorem, and conjectured and proven properties of asymptotic shapes. We finish by discussing the rate of convergence to the limit shape, along with definitions of scaling exponents and a sketch of the proof of the KPZ scaling relation.

==> macros.tex <==
%    If you need symbols beyond the basic set, uncomment this command.
\usepackage{amssymb}

%    If your article includes graphics, uncomment this command.
%\usepackage{graphicx}

%    If the article includes commutative diagrams, ...
%\usepackage[cmtip,all]{xy}

%    Include other referenced packages here.
\usepackage{amsmath,amsthm,tikz,mathrsfs,pgfplots,enumerate}
\usepackage{bm}
%\usepackage{subfiles}
\RequirePackage[numbers,sort&compress]{natbib}
\RequirePackage{color}
\definecolor{my-link}{rgb}{0.5,0.0,0.0}
\definecolor{my-blue}{rgb}{0.0,0.0,0.6}
\definecolor{my-red}{rgb}{0.5,0.0,0.0}
\definecolor{my-green}{rgb}{0.0,0.5,0.0}
\RequirePackage[colorlinks, urlcolor=my-blue,linkcolor=my-link,citecolor=my-green]{hyperref}
%\usepackage[colorlinks=true]{hyperref}
%the link colors were adjusted slightly so that they print nicely even in black and white

%\usepackage[left=1in,top=1in,right=1in,bottom=1in]{geometry}
%\usepackage[left=1.5in,top=1.5in,right=1.5in,bottom=1.4in]{geometry}

%\linespread{1.1}     %this works nicely to produce a more readable cropped 2-1
\usepackage{scalerel}    %%%%  used first for scaling \bullet  
\usepackage{stmaryrd}   %%%% for integer interval notation 
\usepackage{mathabx}   %% made \widecheck work  
\usepackage{hyphenat}

\usepackage{afterpage}

\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\renewcommand{\bibsection}{\section*{\refname}}

%Ivan's packages
\usepackage{bbm}
%\usepackage{amsfonts,amsbsy, amscd}
%\usepackage{graphicx,psfrag,subfigure} %,url}
%\usepackage{cite}
%\usepackage[DIV13]{typearea}
%\usepackage{comment}
%\usepackage{caption}
%\usepackage{setspace}
%\usepackage{float}

%\usepackage{chapterbib}
%\usepackage{minitoc}
%\usepackage{appendix}
%\setcounter{secnumdepth}{3}

%\usepackage{filemod} 
%\date{Last modified on \today\ at\ \filemodprinttime{\jobname}}
%\date{December 05, 2016}



%    Update the information and uncomment if AMS is not the copyright
%    holder.
%\copyrightinfo{2009}{American Mathematical Society}

\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{formal}[theorem]{Critical point derivation}
\newtheorem{experiment}[theorem]{Experimental Result}
\newtheorem{clam}[theorem]{Claim}

\theoremstyle{definition}
\newtheorem{definition}[theorem]{Definition}
\newtheorem{example}[theorem]{Example}
%\newtheorem{xca}[theorem]{Exercise}
\newtheorem{exercise}[theorem]{Exercise}
\newtheorem{assumption}[theorem]{Assumption}
\newtheorem{conj}[theorem]{Conjecture}

\theoremstyle{remark}
\newtheorem{remark}[theorem]{Remark}
\newenvironment{remarks}{\begin{remark}\normalfont}{\end{remark}}
\newtheorem{quest}{Question}


\allowdisplaybreaks[1]
\numberwithin{figure}{section}
\numberwithin{equation}{section}

\newcommand\docname[2]{#2}

\let\LATEXindex\index % save old definition to prevent recursion
\renewcommand\index[1]{\LATEXindex{#1|docname{\jobname}}}
\makeindex

%%%%%%%%%%%%%%%%%%%%
%Firas' macros
%%%%%%%%%%%%%%%%%%%%
\definecolor{sussexg}{rgb}{0,0.7,0.7}
\definecolor{sussexp}{rgb}{0.4,0,0.4}
\definecolor{sussexb}{rgb}{0.4,0.4,0.7}
\definecolor{mygray}{rgb}{0.75,0.75,0.75}


\newcommand{\E}{\mathbb{E}}
\newcommand{\cG}{\mathcal{G}}
\newcommand{\cA}{\mathcal{A}}
\newcommand{\cC}{\mathcal{C}}
\newcommand{\cH}{\mathcal{H}}
\newcommand{\cN}{\mathcal{N}}
\newcommand{\cM}{\mathcal{M}}
\newcommand{\cB}{\mathcal{B}}
\newcommand{\cT}{\mathcal{T}}
\renewcommand{\P}{\mathbb{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Q}{\mathbb{Q}}
\newcommand{\Z}{\mathbb{Z}}
\newcommand{\N}{\mathbb{N}}
\newcommand{\cF}{\mathcal{F}}
\newcommand{\e}{\varepsilon}
\newcommand{\kS}{\mathfrak{S}}
\def\w{\omega}
\def\Bavg{\overline B}
\def\Gbar{\overline G}
\def\cid{\xi^*}

\def\esssup{\mathop{\mathrm{ess\,sup}}}
\def\range{\mathcal R}
\def\Uset{\mathcal U}
\def\riUset{\Uset^\circ}

\font \mymathbb = bbold10 at 11pt
\newcommand{\one}{\mbox{\mymathbb{1}}}    %indicator function

\def\thick{2pt}



%%%%%%%%%%%%%%%%%%%%
%Timo's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\be}{\begin{equation}}
\newcommand{\ee}{\end{equation}}
\newcommand{\beq}{\begin{equation}}
\newcommand{\eeq}{\end{equation}}
\newcommand{\nn}{\nonumber}
\providecommand{\abs}[1]{\vert#1\vert}
\newcommand{\fl}[1]{\lfloor{#1}\rfloor} 
\newcommand{\ce}[1]{\lceil{#1}\rceil}
\def\cC{\mathcal{C}}  \def\cD{\mathcal{D}}
\def\cR{\mathcal{R}}
\def\cU{\mathcal{U}}
\def\cK{\mathcal{K}}
\def\cX{\mathcal{X}}\def\cY{\mathcal{Y}}\def\cZ{\mathcal{Z}}
\def\bE{\mathbb{E}} \def\bL{\mathbb{L}}
\def\uvec{\mathbf{u}}\def\vvec{\mathbf{v}}
\def\wvec{\mathbf{w}}
\def\ind{\mathbf{1}}
\def\ddd{\displaystyle} 
\def\Vvv{{\rm\mathbb{V}ar}}  \def\Cvv{{\rm\mathbb{C}ov}} 
\def\wt{\widetilde}  \def\wh{\widehat} \def\wb{\overline} \def\wc{\widecheck}
\def\north{S_{\mathcal N}}  \def\south{S_{\mathcal S}}  \def\east{S_{\mathcal E}}  
\def\west{S_{\mathcal W}}  
\def\OSP{(\Omega, \kS, \P)}
\def\Gpl{G}
\def\Gpp{G}
\def\gpp{g_{\text{\rm pp}}}
\def\gpl{g_{\text{\rm pl}}}  
\def\B{{B}}
\DeclareMathOperator{\dist}{dist}
\DeclareMathOperator{\Var}{Var}
\DeclareMathOperator{\ri}{ri}    %rel interior  
\DeclareMathOperator{\conv}{co}   %convex hull  
\def\sigmawc{\wc\sigma}   %sigma check (needed version that doesn't start \w...  
\def\loexp{\chi}  %longitudinal exponent
\def\trexp{\zeta}  %transverse exponent
\def\deq{\overset{d}=} 
\def\qedex{\hfill$\triangle$} 
\def\bincr{B}   \def\tincr{t}   \def\Iincr{I}
\def\Xw{X}  %another letter for a weight 
\def\Yw{Y}  %another letter for a weight 
\def\ul{\underline}  
\def\exitt{\tau} %exit time from axis 
\def\Gppo{{{}^o\Gpp}}
\newcommand\bbullet{{\raisebox{0.5pt}{\scaleobj{0.6}{\bullet}}}} %% looks good for paths x_\bbullet 
\newcommand\brbullet{{\raisebox{-1pt}{\scaleobj{0.5}{\bullet}}}} %%  for subscript paths x_\bbullet   need negative raise 
\newcommand\cbullet{{\raisebox{1pt}{\scaleobj{0.6}{\bullet}}}}
\newcommand\dbullet{{\scaleobj{0.7}{\bullet}}}   % same as \bbullet but without shift up


%%%%%%%%%%%%%%%%%%%%
%Ivan's macros
%%%%%%%%%%%%%%%%%%%%
\newcommand{\bflambda}{\ensuremath{\bar{\lambda}}}
\newcommand{\bfmu}{\ensuremath{\bar{\mu}}}
\newcommand{\bfnu}{\ensuremath{\bar{\nu}}}
\newcommand{\I}{{\rm i}}
\newcommand{\Id}{\mathbbm{1}}
\newcommand{\Or}{\mathcal{O}}
%\newcommand{\e}[0]{\varepsilon}
\newcommand{\BesselK}{\ensuremath{\mathrm{K}}}
\newcommand{\EE}{\ensuremath{\mathbb{E}}}
\newcommand{\PP}{\ensuremath{\mathbb{P}}}
%\newcommand{\R}{\ensuremath{\mathbb{R}}}
\newcommand{\C}{\ensuremath{\mathbb{C}}}
%\newcommand{\Z}{\ensuremath{\mathbb{Z}}}
\newcommand{\Rplus}{\ensuremath{\mathbb{R}_{+}}}
\newcommand{\Zgzero}{\ensuremath{\mathbb{Z}_{>0}}}
\newcommand{\Zgeqzero}{\ensuremath{\mathbb{Z}_{\geq 0}}}
\newcommand{\Zleqzero}{\ensuremath{\mathbb{Z}_{\leq 0}}}
%\newcommand{\Q}{\ensuremath{\mathbb{Q}}}
\newcommand{\Y}{\ensuremath{\mathbb{Y}}}
\newcommand{\M}{\ensuremath{\mathbf{M}}}
\newcommand{\MM}{\ensuremath{\mathbf{MM}}}
\newcommand{\W}[1]{\ensuremath{\mathbf{W}}_{(#1)}}
\newcommand{\WM}[1]{\ensuremath{\mathbf{WM}}_{(#1)}}
\newcommand{\Zsd}{\ensuremath{\mathbf{Z}}}
\newcommand{\Fsd}{\ensuremath{\mathbf{F}}}
\newcommand{\Usd}{\ensuremath{\mathbf{U}}}
\newcommand{\Sym}{\ensuremath{\mathrm{Sym}}}
\newcommand{\Gdist}{\ensuremath{\mathrm{Gamma}}}
\newcommand{\LogGdist}{\ensuremath{\log\Gamma}}
\newcommand{\Hi}{\ensuremath{\mathcal{H}}}
\newcommand{\Res}[1]{\underset{{#1}}{\mathrm{Res}}}
\newcommand{\ta}[0]{\varphi}
\newcommand{\T}{\mathbb{T}}
\newcommand{\la}{\lambda}
\newcommand{\ga}{\gamma}
\newcommand{\ep}{\epsilon}
\newcommand{\RR}{\mathbb{R}_+\times\mathbb{R}}

\renewcommand{\d}{\mathrm d}
\renewcommand{\Re}{\operatorname{Re}}
\renewcommand{\Im}{\operatorname{Im}}
\DeclareMathOperator{\tr}{Tr}
\DeclareMathOperator{\Ai}{Ai} \DeclareMathOperator{\sign}{sgn}
\DeclareMathOperator*{\var}{Var}
\DeclareMathOperator*{\sgn}{sgn}




%%%%%%%%%%%%%%%%%%%%
%Jack's macros
%%%%%%%%%%%%%%%%%%%%

%commands
\newcommand{\prob}{\mathbf{P}}
%\newcommand{\Z}{\mathbb{Z}}
\newcommand{\cE}{\mathcal{E}}
%\newcommand{\cB}{\mathcal{B}}
%\newcommand{\cN}{\mathcal{N}}
\newcommand{\bfE}{\mathbf{E}}
\newcommand{\bbS}{\mathbb{S}}
\newcommand{\bbR}{\mathbb{R}}


